A Local-to-Global Approach to Multi-modal Movie Scene Segmentation

Scene, as the crucial unit of storytelling in movies, contains complex activities of actors and their interactions in a physical environment. Identifying the composition of scenes serves as a critical step towards semantic understanding of movies. This is very challenging -- compared to the videos studied in conventional vision problems, e.g. action recognition, as scenes in movies usually contain much richer temporal structures and more complex semantic information. Towards this goal, we scale up the scene segmentation task by building a large-scale video dataset MovieScenes, which contains 21K annotated scene segments from 150 movies. We further propose a local-to-global scene segmentation framework, which integrates multi-modal information across three levels, i.e. clip, segment, and movie. This framework is able to distill complex semantics from hierarchical temporal structures over a long movie, providing top-down guidance for scene segmentation. Our experiments show that the proposed network is able to segment a movie into scenes with high accuracy, consistently outperforming previous methods. We also found that pretraining on our MovieScenes can bring significant improvements to the existing approaches.

==> articles/application.tex <==
% !TEX root = ../main.tex

\section{Extension}
\label{sec:application}
Segmented scene can facilitate a variety of applications, with which we can step further into high-level semanic understandings. Three potential usages are listed in this section, namely 1) improving movie character recognition; 2) generating human interaction graph; and 3) facilitating scene retrieval across movies. More advanced tasks based on scenes will be explored in future works.
% 1

\textbf{Movie character recognition} is a challenging task because many figures in a movie shot show up without the full faces.
Segmented scene help reduce the search space, given that the set of characters appeared within one scene must be the same. The character without full face is likely to be the one shown up with faces in any other part of the same scene.


% 2
\textbf{Human interaction graph} can be used to study the evolution of plot and characters' relationships in a movie, which is important for high-level movie understandings. For example, based on the segmented Scenes, we can count the total time of interaction between different character pairs. Then we can infer the importance of different characters in different movie parts, and how the story evolves.

% 3
In the task of \textbf{Cross Movie Scenario Retrieval}, a certain scene is given and we are asked to retrieve similar ones in other movies. For example, given a scene of ``people chatting in a room", we would like to retrieve all the similar scenes (chatting) from other movies. This task is of great practical interest and has a variety of real-world applications. It requires a semanic understanding of videos that goes beyond recognizing the visual appearance or simple
action pattern. Compared to a single shot, the segmented scenes allows us to extract rich correlated features (\eg~characters, specific objects,
and places) in a self-contained semantic segment. 

The aforementioned three examples are only a brief introduction to the potential usage of segmented scenes. There remains much more tasks and open problems could be built upon segmented scenes, especially those contributing to the high-level movie understandings.
